Driving Behavior Explanation with Multi-level Fusion

In this era of active development of autonomous vehicles, it becomes crucial to provide driving systems with the capacity to explain their decisions. In this work, we focus on generating high-level driving explanations as the vehicle drives. We present BEEF, for BEhavior Explanation with Fusion, a deep architecture which explains the behavior of a trajectory prediction model. Supervised by annotations of human driving decisions justifications, BEEF learns to fuse features from multiple levels. Leveraging recent advances in the multi-modal fusion literature, BEEF is carefully designed to model the correlations between high-level decisions features and mid-level perceptual features. The flexibility and efficiency of our approach are validated with extensive experiments on the HDD and BDD-X datasets.

==> tables/bdd/bdd_sample_short.tex <==
\begin{table*}%[b]
    \centering
    \caption{\textbf{Samples of generated explanations}.}
    %A decoding temperature of $0.3$ has been used to encourage diversity.}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}l l l@{}}
        \toprule
        Human (gold-label) & Generated by \acro{} (greedy) & Generated by \acro{} (temperature=0.3)\\
        %\fontsize{11}{11}{\selectfont Human (gold-label)} & \fontsize{11}{11}{\selectfont Generated by \acro{}} \\
        \hline
        % Driving forward
        %because the light is green and the intersection is clear & because the light is green \\        % Green light
        after the light turned green and traffic accelerates & because the light turns green & because the light has turned green \\ % Green light -- LINE 74
        %because there are no nearby cars in front of it & as the lane is clear ahead \\ % lane is clear
        because traffic is moving at a steady speed & because traffic is moving at a steady speed & as traffic ahead is moving steadily \\ % Steady speed -- LINE 239
        
        % SLOWING
        %as it approaches slower moving traffic in front of it & as the car in front of it slows \\ % traffic slows
        because it is approaching a red stop sign & \eloih{because the light is red} & as it approaches a stop sign \\ %stop sign -- LINE 283
        
        % STOPPING
        %because there is a stop sign & because there is a stop sign at the intersection \\ %stop sign
        %traffic ahead is stopping at an intersection & as traffic ahead is stopped \\ % congestion
        since the light is red and there are pedestrians crossing & \eloih{because the light is red} & as the light is red and pedestrians are crossing the street \\ % red light and people -- LINE 1565
        %because the light is red and there are cars and people crossing & because the light is red and pedestrians are crossing the street \\ % red light
        
        % DEVIATION
        since there was a stopped vehicle in the way & \eloih{because the lane is clear} & to get around a car parked in its lane \\ % -- LINE 219
        
        
%        \multicolumn{2}{c}{Action = \textit{The car stopped}} \\
%since the light is red and there are people crossing the road	&	because the light is red	\\
%for the red light	&	because the light is red	\\
%because the van in front was'nt moving	&	because traffic is stopped	\\
%because the van stopped moving	&	because traffic is stopped	\\
%because the light has'nt turned green yet	&	because the light is red	\\
%since there is a stop just ahead	&	because there is a stop sign	\\
%when traffic in front of it stops	&	because the car in front of it is stopped	\\
%
%        \hline
%        \multicolumn{2}{c}{Action = \textit{The car slows}} \\
%
%since the van started moving	&	because traffic is moving slowly	\\
%because the van in front is moving at different speeds	&	because traffic is moving slowly	\\
%
%        \hline
%        \multicolumn{2}{c}{Action = \textit{The car drives forward}} \\
%
%because the light is green and the intersection is clear	&	because the light is green	\\
%because there are no nearby cars in its lane impeding it	&	because the road is clear	\\
%because the pedestrians had moved out of the way	&	because the road is clear	\\
%since the street is clear of traffic	&	because the road is clear	\\
%
%        \hline
%        \multicolumn{2}{c}{Action = \textit{The car accelerates}} \\
%
%because traffic is now moving in both lanes	&	because traffic is moving forward	\\
%because the traffic ahead starts moving faster	&	because traffic is moving forward	\\
%
%        \hline
%        \multicolumn{2}{c}{Action = \textit{The car turns right}} \\
%
%since it is allowed to turn right	&	because it s turning to the right	\\


        
%since there are many obstacles to be aware of	&	because traffic is moving at a steady speed	\\
%since the light ahead became red	&	because the light turned green	\\
%since the light is red and there are people crossing the road	&	because the light is red	\\
%because the lights are green and there is little traffic	&	because the road is clear	\\
%because the traffic ahead starts moving faster	&	because traffic is moving forward	\\
%because there are no nearby cars in its lane and the light is green	&	because the road is clear	\\
%as it prepares to make a left hand turn	&	because there is a stop sign	\\
%to enter another road while the light is green	&	because the road is clear	\\
%because there are no nearby cars in its lane impeding it	&	because the road is clear	\\
%for the red light and a pedestrian in the crosswalk	&	because the light ahead is red	\\
%for the red light	&	because the light is red	\\
%because there are cars and people nearby	&	because traffic is moving at a steady speed	\\
%because the car can turn right	&	because the road is clear	\\
%to avoid the car in front on the left	&	because the road is clear	\\
%because there are pedestrians blocking the path to the right	&	because there is a stop sign	\\
%since it is waiting for the pedestrians to cross	&	because there is a stop sign	\\
%because the pedestrians had moved out of the way	&	because the road is clear	\\
%since the car had just turned right	&	because the road is clear	\\
%because traffic is now moving in both lanes	&	because traffic is moving forward	\\
%because traffic is moving forward	&	because the car in front is slowing down	\\
%because traffic is moving faster in that lane	&	because the lane is clear	\\
%because now that lane is moving faster	&	because the car in front is slowing down	\\
%because traffic is moving slowly	&	because traffic is moving at a steady speed	\\
%because the cars ahead have stopped	&	because the light is red	\\
%because the van in front was nt moving	&	because traffic is stopped	\\
%since the van started moving	&	because traffic is moving slowly	\\
%because the van stopped moving	&	because traffic is stopped	\\
%because the van in front is moving at different speeds	&	because traffic is moving slowly	\\
%as traffic in front of it moves slowly and merges together	&	because the car in front of it is moving forward	\\
%when traffic in front of it stops	&	because the car in front of it is stopped	\\
%as traffic in front of it moves forward slightly	&	because the car in front of it has stopped	\\
%because there are no nearby cars in its lane	&	because the car in front of it has slowed down	\\
%while there is a gap in traffic	&	because the car in front is moving forward	\\
%because there are no nearby cars in front of it	&	because the car in front is moving forward at a normal speed	\\
%because the light has nt turned green yet	&	because the light is red	\\
%because there was no incoming traffic to block it from turning left	&	because the road is clear	\\
%because it is trying to pass the yellow light quickly	&	because the road is clear	\\
%since there is a stop just ahead	&	because there is a stop sign	\\
%because it is trying to be safe	&	because there is a stop sign	\\
%since it is allowed to turn right	&	because it s turning to the right	\\
%since there are cars close to it	&	because the road is clear	\\
%because the light is green and the intersection is clear	&	because the light is green	\\
%since the street is clear of traffic	&	because the road is clear	\\
        \bottomrule
    \end{tabular}
    }
    \label{tab:bdd_sample_short}
\end{table*}

==> tables/blinker.tex <==
\begin{table*}[t]
    \centering
    \caption{\textbf{Comparison to state-of-the-art on the \textit{cause} labels of \hdd{}.} % Models are trained on \hdd{} train split and the results are computed on the test split.
    Results in bold are the best among \textit{online} models. For the sake of completeness, we also report performance of offline models.}
    \begin{tabular}{@{}r@{\hspace{0.2cm}}ccccccc@{\hspace{0.35cm}}c@{}}
    \toprule
    \noalign{\vspace{-0.09cm}}
    & \multicolumn{6}{c}{\ffz{Individual causes}} & \\
    \cline{2-7}
    System & \fz{Congest.} & \fz{Sign} & \makecell[b]{\fz{Red} \\\fz{light}} & \makecell[b]{\fz{Crossing} \\ \fz{vehicle}} & \makecell[b]{\fz{Parked} \\ \fz{vehicle}} & \makecell[b]{\fz{Crossing} \\ \fz{pedestrian}} & \makecell[b]{Overall \\ mAP} & \makecell[b]{Driver \\ MSE} \\
    \noalign{\smallskip}
    Multi-head  & 81.25 & 66.59 & 75.46 & 31.21 & 10.24 & 25.62 & 48.39 & 1.36 \\ 
    Multi-head + blinker & 72.56 & \textbf{66.68} & \textbf{83.22} & 38.38 & \textbf{14.88} & 24.15 & 49.98 & 1.39 \\
    \acro{} no blinker & \textbf{82.29} & 63.40 & 79.47 & 38.48 & 12.01 & 16.77 & 48.74 & 1.39 \\
    \acro{} & 80.38 & 63.41 & 81.94 & \textbf{41.19} & 12.18 & \textbf{27.19} & \textbf{50.96} & \textbf{1.33} \\
    \bottomrule
    \end{tabular}
    %}
    \label{tab:blinker}
\end{table*}

==> tables/fusion_choice.tex <==

\begin{table}[t]
    \centering
    \caption{Comparing different fusion methods for a fusion between Prediction and Layer2. Trained on mini-train, results on mini-val}
    \begin{tabular}{@{}lccccc@{}}
    %\hline
    \toprule
    Fusion model & Concat+MLP & Bilinear & Tucker & MUTAN & BLOCK \\
    \hline
     mAP & 28.15\fontsize{6}{6}{\selectfont$\pm$0.72} & 16.71\fontsize{6}{6}{\selectfont$\pm$0.77} & 27.72\fontsize{6}{6}{\selectfont$\pm$0.36} & 27.70\fontsize{6}{6}{\selectfont$\pm$0.32} & 28.90\fontsize{6}{6}{\selectfont$\pm$0.89}\\
     mAP & 28.50\fontsize{6}{6}{\selectfont$\pm$0.52} & 16.31\fontsize{6}{6}{\selectfont$\pm$0.47} & 27.60\fontsize{6}{6}{\selectfont$\pm$0.41} & 27.51\fontsize{6}{6}{\selectfont$\pm$0.11} & 29.41\fontsize{6}{6}{\selectfont$\pm$0.21} \\
    \bottomrule 
    \end{tabular}
    \label{tab:fusion_choice}
\end{table}
